Revisiting Block-based Quantisation: What is Important for Sub-8-bit LLM Inference?

The inference of Large language models (LLMs) requires immense computation and memory resources. To curtail these costs, quantisation has merged as a promising solution, but existing LLM quantisation mainly focuses on 8-bit. In this work, we explore the statistical and learning properties of the LLM layer and attribute the bottleneck of LLM quantisation to numerical scaling offsets. To address this, we adapt block quantisations for LLMs, a family of methods that share scaling factors across packed numbers. Block quantisations efficiently reduce the numerical scaling offsets solely from an arithmetic perspective, without additional treatments in the computational path. Our nearly-lossless quantised 6-bit LLMs achieve a $19\times$ higher arithmetic density and $5\times$ memory density than the float32 baseline, surpassing the prior art 8-bit quantisation by $2.5\times$ in arithmetic density and $1.2\times$ in memory density, without requiring any data calibration or re-training. We also share our insights into sub-8-bit LLM quantisation, including the mismatch between activation and weight distributions, optimal fine-tuning strategies, and a lower quantisation granularity inherent in the statistical properties of LLMs. The latter two tricks enable nearly-lossless 4-bit LLMs on downstream tasks. Our code is open-sourced.

==> archived/accuracy_data.tex <==



==> archived/cost_model_ad.tex <==
\begin{tikzpicture}[thick,scale=0.9, every node/.style={scale=0.9}]
\pgfplotsset{every x tick label/.append style={font=\footnotesize}, compat=1.3}
\tikzset{>=latex}
\begin{axis}[
    height=70mm,
    width=80mm,
    xlabel={\footnotesize Normalised memory density to Float32},
    ylabel={\footnotesize Normalised arithmetic density to Float32},
    ylabel style = {align=center},
    xmin=0, ymin=0.8, ymax=32, xmax=35,
    % , xmax=32, ymax = 32, ymin = 0.0004,
    % xtick={0, 5, 10, 15, 20, 25, 30},
    ytick={1, 2, 4, 8, 16, 32},
    ymode=log, log ticks with fixed point,
    scaled x ticks = false, 
    scaled y ticks = false,
    legend columns = 2,
    legend style={at={(0.4,0.2)},anchor=west, draw=none, fill=none, font=\footnotesize},
    legend cell align={left},
    ]

\addplot[jcgreen, draw=jcgreen, mark=triangle, draw=none] table
[x=md, y=ad, col sep=space] {bfp.dat};
\addlegendentry{BFP}

\addplot[jcbrown, draw=jcbrown, mark=oplus, draw=none] table
[x=md, y=ad, col sep=space] {bl.dat};
\addlegendentry{BL}

\addplot[jcpurple, draw=jcpurple, mark=square, draw=none] table
[x=md, y=ad, col sep=space] {bmf.dat};
\addlegendentry{BM}

\addplot[draw=jcblue, mark=*, fill=jcblue] coordinates {(1, 1)};
\addlegendentry{Float32}

\addplot[draw=jcorange, mark=diamond*, fill=jcorange] coordinates {(4, 7.66)};
\addlegendentry{Int8}

\addplot[draw=jcred, mark=star, fill=jcred] coordinates {(4, 17.4)};
\addlegendentry{MiniFloat}

\addplot[->, black, line width = 1pt] coordinates {(26, 28) (34, 28)};
\addplot[->, black, line width = 1pt] coordinates {(34, 12) (34, 26)};
\node[black] at (axis cs: 24, 26) {good};
\node[black] at (axis cs: 32, 10) {good};

\end{axis}
\end{tikzpicture}


==> archived/cost_model_lut.tex <==
\begin{tikzpicture}[thick,scale=0.9, every node/.style={scale=0.9}]
\pgfplotsset{every x tick label/.append style={font=\footnotesize}, compat=1.3}
\begin{axis}[
    height=70mm,
    width=80mm,
    xlabel={\footnotesize Effective bit width},
    ylabel={\footnotesize Normalised Area},
    ylabel style = {align=center},
    % xmin=0, xmax=32, ymax = 32, ymin = 0.0004,
    % xtick={0, 5, 10, 15, 20, 25, 30},
    % ytick={5e-4, 0.001, 0.01, 0.1, 0.25, 0.5, 1, 2, 4, 8, 16, 32},
    % ymode=log, log ticks with fixed point,
    scaled x ticks = false, 
    scaled y ticks = false,
    % legend columns = 5,
    legend style={at={(0.05,0.78)},anchor=west, draw=none, fill=none, font=\footnotesize},
    legend cell align={left},
    ]

\addplot[jcgreen, draw=jcgreen, mark=triangle, draw=none] table
[x=eb, y=lut, col sep=space] {bfp.dat};
\addlegendentry{Block Floating Point}

\addplot[jcbrown, draw=jcbrown, mark=oplus, draw=none] table
[x=eb, y=lut, col sep=space] {bl.dat};
\addlegendentry{Block Logarithm}

\addplot[jcpurple, draw=jcpurple, mark=square, draw=none] table
[x=eb, y=lut, col sep=space] {bmf.dat};
\addlegendentry{Block MiniFloat}

\addplot[draw=jcblue, mark=*, fill=jcblue] coordinates {(32, 835)};
\addlegendentry{Float32}

\addplot[draw=jcorange, mark=diamond*, fill=jcorange] coordinates {(8, 109)};
\addlegendentry{Int8}

\addplot[draw=jcred, mark=star, fill=jcred] coordinates {(8, 48)};
\addlegendentry{MiniFloat}

\end{axis}
\end{tikzpicture}


==> archived/layerwise_qkv_bits.tex <==



==> archived/lut_data.tex <==








==> archived/precision_compare.tex <==
\begin{tikzpicture}[thick,scale=0.9, every node/.style={scale=0.9}]
\pgfplotsset{every x tick label/.append style={font=\footnotesize}, compat=1.3}
\begin{axis}[
    height=70mm,
    width=80mm,
    xlabel={\footnotesize Values in binary},
    ylabel={\footnotesize Values in float},
    ylabel style = {align=center},
    % xmin=0, xmax=32, ymax = 32, ymin = 0.0004,
    % xtick={0, 5, 10, 15, 20, 25, 30},
    ytick={0.125, 0.25, 0.5, 1, 2, 4, 8},
    ymode=log, 
    log ticks with fixed point,
    scaled x ticks = false, 
    scaled y ticks = false,
    % legend columns = 5,
    legend style={at={(0.04,0.88)},anchor=west, draw=none, fill=none, font=\footnotesize},
    legend cell align={left},
    ]

\addplot[jcblue, draw=jcblue, mark=none, line width=1pt] table
[x=x, y=denorm, col sep=space] {prec.dat};
\addlegendentry{DMF}

\addplot[jcred, draw=jcred, mark=none, line width=1pt] table
[x=x, y=norm, col sep=space] {prec.dat};
\addlegendentry{MiniFloat}

\end{axis}
\end{tikzpicture}


==> archived/precision_data.tex <==



==> archived/ptq_vs_taq_downstream.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcrrrr}
\toprule
\multicolumn{1}{c}{Task} & \multicolumn{1}{c}{Quantisation} & Fine-Tune Style & \multicolumn{1}{c}{Zero-shot prompting} & \multicolumn{1}{c}{Epoch 1} & \multicolumn{1}{c}{Epoch 2} & \multicolumn{1}{c}{Epoch 3} \\ \midrule
SST2 & FP32 & - & 82.2 & 93.9 & 93.2 & 94.0 \\
 & 4-bit BFP & PTQ on fine-tuned FP32 & \multirow{2}{*}{58.1 (-24.1)} & 93.7 (-0.2) & 93.2 (0) & 93.6 (-0.5) \\
 & 4-bit BFP & TAQ on downstream &  & 94.3 (+0.4) & 94.2 (+0.9) & 94.2 (+0.1) \\ \midrule
QNLI & FP32 & - & 51.3 & 89.0 & 90.6 & 91.7 \\
 & 4-bit BFP & PTQ on fine-tuned FP32 & \multirow{2}{*}{50.2 (-1.1)} & 86.6 (0.5) & 89.1 (-1.5) & 90.3 (-1.4) \\
 & 4-bit BFP & TAQ on downstream &  & 86.6 (-2.5) & 89.7 (-0.9) & 91.0 (-0.7) \\ \bottomrule
\end{tabular}}
\caption{
Accuracy ($\uparrow$) comparison between PTQ on fine-tuned FP32 and TAQ on downstream of 4-bit LLM. We compare these two styles on the tasks where FP32 zero-shot prompting LLM performs poorly. Both two options improve the accuracy effectively, aligning quantised LLMs' accuracy with FP32.
}
\label{tab:ptq_vs_taq_downstream}
\end{table*}

==> archived/taq_on_wikitext2.tex <==
\begin{table*}[]


\centering

\begin{tabular}{cccccc}
\toprule
Method   
& Float32 
& Fixed-point 
& MiniFloat 
& DMF 
& BFP
% & BFP-mixed 
\\ 
Config   
& - 
& W8A8 
& W8A8 
& W8A8
& W4.5A4.5
% & W3.5A3.5   
\\ 
\midrule
OPT-125M 
& 27.3    
& 61.1 ($+34.3$)            
& 29.8 ($+ 2.5$)    
& 30.1 ($+ 2.8$)         
& 34.3 ($+7.0$)  
% & 33.7 ($+6.4$)
\\
OPT-350M 
& 23.4    
& 36.3 ($+12.9$)            
& 23.5($+0.1$)    
& 24.4 ($+ 1.1$)          
& 26.3 ($+2.9$)   
% & 30.7 ($+7.3$) 
\\
Mem $\uparrow$
& 1$\times$
& 4$\times$         
& 4$\times$   
& 4$\times$        
& 7.1 $ \times$  
% & 9.1 $ \times$
\\
Arith $\uparrow$
& 1$\times$   
& 7.7$\times$          
& 17.4$\times$    
& 17.4$\times$          
& 37.3$\times$   
% & $\times$ 
\\
\bottomrule
\end{tabular}
\caption{Perplexity ($\downarrow$) values with TAQ on WikiText2, this means we directly quantise the pre-trained model and then fine-tune with quantisation on WikiText2. Mem and Airth represent Memory and Arithmetic density accordingly. DMF, BFP and BFP-mixed represent Denormalised MiniFloat, Block Floating Point and Block Floating Point with mixed precisions respectively.}
% \label{tab:opt_taq}
\end{table*}

==> images/1_Introduction/bk_motivation.tex <==

\begin{figure*}[!t]
\centering
\begin{minipage}[b]{.4\linewidth}
\begin{algorithm}[H]
\caption{Transformer layer}
\begin{algorithmic}[1]
\footnotesize
\Require $X$ \Comment{Input features}
\Require $H$ \Comment{Number of heads}
\Require $L$ \Comment{Number of hidden layers}
\State $\capped{X_n} \gets LayerNorm(X) $
\For{$i \in [0, H)$}
\State $\varied{Q_i} \gets \capped{X_n}W_{Q_i} $
\myflushright{\textcircled{\small{1}}}

\State $\varied{K_i} \gets \capped{X_n}W_{K_i} $
\myflushright{\textcircled{\small{2}}}

\State $\varied{V_i} \gets \capped{X_n}W_{V_i} $
\myflushright{\textcircled{\small{3}}}

\State $A_i \gets \frac{\varied{Q_i}\varied{K_i^T}}{\sqrt{d_k}} $
\myflushright{\textcircled{\small{4}}}

\State $\capped{\hat{A}_i} \gets softmax(A_i, axis \gets -1) $

\State $B_i \gets \capped{\hat{A}_i}\varied{V_i} $
\myflushright{\textcircled{\small{5}}}

\EndFor
\State $\varied{B_c} \gets concat(B_0..B_{L-1})$

\State $B_0 \gets \varied{B_c}W_0+b_0$
\myflushright{\textcircled{\small{6}}}

\State $\capped{B_n} \gets LayerNorm(B_0 + \capped{X_n}) $

% \State $\varied{B_1} \gets \max{(0, \capped{B_n} W_1+b_1)} $
\State $\varied{B_1} \gets act(\capped{B_n} W_1+b_1)) $
\myflushright{\textcircled{\small{7}}}

\State $B_2 \gets \varied{B_1}W_2+b_2 $
\myflushright{\textcircled{\small{8}}}

\State $O \gets B_2 + B_n$
\State \Return $O$
\end{algorithmic}
\label{alg:transformer}
\end{algorithm}
\end{minipage}
\begin{minipage}[b]{.55\linewidth}
\input{images/1_Introduction/figure_6.7b_act}
\end{minipage}
\caption{The algorithm on the left is the forward pass computation of a single Transformer layer \cite{vaswani2017attention} in mainstream LLMs, wherein values in \textcolor{jcblue}{blue} (\textit{e.g.}\textcolor{jcblue}{$X_n$}) represent tensors with predetermined min-max values, such as the outputs of a normalisation layer or softmax. Values in \textcolor{jcred}{red} have unbounded min-max, and are plotted on the upper right for different layers of OPT-6.7B \cite{zhang2022opt} on Wikitext2. The plot on the lower right depicts the weight variance. We show that for almost all of these tensors, their variances increase at deeper layers, resulting in \emph{scaling offsets} in their quantizations.}
\label{fig:introduction:motivation}
\end{figure*}


==> images/1_Introduction/figure_6.7b_act.tex <==
\begin{tikzpicture}[thick,scale=0.95, every node/.style={scale=0.95}]
\pgfplotsset{every x tick label/.append style={font=\footnotesize}, compat=1.3}
\begin{axis}[
    height=45mm,
    width=80mm,
    xlabel={\footnotesize Layer ID},
    ylabel={\footnotesize Variance},
    ylabel style = {align=center},
    xmin=0, xmax=32, ymax = 32, ymin = 0.0004,
    xtick={0, 5, 10, 15, 20, 25, 30},
    ytick={5e-4, 0.001, 0.01, 0.1, 0.25, 0.5, 1, 2, 4, 8, 16, 32},
    ymode=log, log ticks with fixed point,
    scaled x ticks = false, 
    scaled y ticks = false,
    legend columns = 5,
    ylabel shift=-1em,
    legend style={at={(0,-0.2)},anchor=west, draw=none, fill=none, font=\footnotesize},
    ]

\addplot[jcred, draw=jcred, mark=o, line width=1pt, mark options={scale=0.7}] table
[x=layer, y=q, col sep=space] {data6.7b.dat};
\addlegendentry{$\varied{Q}$}

\addplot[jcblue, draw=jcblue, mark=star, line width=1pt] table
[x=layer, y=k, col sep=space] {data6.7b.dat};
\addlegendentry{$\varied{K}$}

\addplot[jcgreen, draw=jcgreen, mark=square, line width=1pt, mark options={scale=0.7}] table
[x=layer, y=v, col sep=space] {data6.7b.dat};
\addlegendentry{$\varied{V}$}

\addplot[jcorange, draw=jcorange, mark=triangle, line width=1pt] table
[x=layer, y=b0, col sep=space] {data6.7b.dat};
\addlegendentry{$\varied{B_c}$}

\addplot[jcpurple, draw=jcpurple, mark=diamond, line width=1pt, mark options={scale=0.7}] table
[x=layer, y=b1, col sep=space] {data6.7b.dat};
\addlegendentry{$\varied{B_1}$}

\end{axis}
\end{tikzpicture}


==> images/1_Introduction/figure_6.7b_weight.tex <==
\begin{tikzpicture}[thick,scale=0.95, every node/.style={scale=0.95}]
% \pgfplotsset{every x tick label/.append style={font=\footnotesize}, compat=1.3}
\begin{axis}[
    height=45mm,
    width=80mm,
    xlabel={\footnotesize Layer ID},
    ylabel={\footnotesize Variance},
    ylabel style = {align=center},
    xmin=0, xmax=32,
    xtick={0, 5, 10, 15, 20, 25, 30},
    % ytick={3.0517578125e-05, 6.103515625e-05, 0.0001220703125, 0.000244140625, 0.00048828125, 0.0009765625}, % y tick: 2^-15, 2^-14, 2^-13, 2^-12, 2^-11, 2^10   
    % ymode=log, log ticks with fixed point,
    ymode=log,
    log basis y={2},
    scaled x ticks = false, 
    scaled y ticks = false,
    legend columns = 1,
    ylabel shift=-1em,
    y tick label style={/pgf/number format/sci},
    legend style={at={(1,1)},anchor=north west, draw=none, fill=none, font=\footnotesize},
    ]

\addplot[jcred, draw=jcred, mark=*, line width=1pt, mark options={solid, scale=0.7}] table
[x=layer, y=wq, col sep=space] {data6.7b.dat};
\addlegendentry{$\capped{W_Q}$}

\addplot[jcblue, draw=jcblue, mark=star*, line width=1pt, mark options={solid}] table
[x=layer, y=wk, col sep=space] {data6.7b.dat};
\addlegendentry{$\capped{W_K}$}

\addplot[jcgreen, draw=jcgreen, mark=square*, line width=1pt, mark options={solid, scale=0.7}] table
[x=layer, y=wv, col sep=space] {data6.7b.dat};
\addlegendentry{$\capped{W_V}$}

\addplot[jcorange, draw=jcorange, mark=triangle*, line width=1pt] table
[x=layer, y=w0, col sep=space] {data6.7b.dat};
\addlegendentry{$\capped{W_0}$}

\addplot[jcpurple, draw=jcpurple, mark=diamond*, line width=1pt, mark options={solid, scale=0.7}] table
[x=layer, y=w1, col sep=space] {data6.7b.dat};
\addlegendentry{$\capped{W_2}$}

\addplot[jcbrown, draw=jcbrown, mark=pentagon*, line width=1pt, mark options={solid, scale=0.7}] table
[x=layer, y=w2, col sep=space] {data6.7b.dat};
\addlegendentry{$\capped{W_1}$}

\end{axis}
\end{tikzpicture}
